Concise and interpretable multi-label rule sets

Multi-label classification is becoming increasingly ubiquitous, but not much attention has been paid to interpretability. In this paper, we develop a multi-label classifier that can be represented as a concise set of simple "if-then" rules, and thus, it offers better interpretability compared to black-box models. Notably, our method is able to find a small set of relevant patterns that lead to accurate multi-label classification, while existing rule-based classifiers are myopic and wasteful in searching rules,requiring a large number of rules to achieve high accuracy. In particular, we formulate the problem of choosing multi-label rules to maximize a target function, which considers not only discrimination ability with respect to labels, but also diversity. Accounting for diversity helps to avoid redundancy, and thus, to control the number of rules in the solution set. To tackle the said maximization problem we propose a 2-approximation algorithm, which relies on a novel technique to sample high-quality rules. In addition to our theoretical analysis, we provide a thorough experimental evaluation, which indicates that our approach offers a trade-off between predictive performance and interpretability that is unmatched in previous work.

==> ack.tex <==
\section{Acknowledgements}
\label{sec:ack}


==> approach.tex <==
\section{Proposed approach}
\label{sec:approach}



==> extensions.tex <==
\section{Extensions}
\label{sec:extens} 


\spara{Two-level classification}
To improve the performance of the proposed rule-based classification approach we could take our idea one step further. 
Once we have learned a set of rules according to the optimization problem discussed in Section~\ref{sec:prob_form} we can assemble a new dataset in which the attributes are merged with the predicted rules. Thus, for each data record we have not only the original items but also the predicted labels. Then, we proceed learning further rules $\ruleset'$ which also fully exploit the label dependencies while avoiding cycles. Clearly the set $\ruleset'$ would complement the original set of learned rules $\ruleset$ in attempt to make the most of the label correlations and predict more labels for each data record which may result in improved accuracy.

\spara{Sampling rare labels}
Our algorithm sample highly co-occurring labels according to the area measure. Clearly, this favours more frequent labels over more rare ones. However, in practice, at prediction time, it would be valuable to cover also less dense regions of the label space. 
In order to achieve this, we can consider a modified area measure, referred to as \emph{weighted} area: 

\begin{equation}
\label{eq:weighted-rel-area}
\wrelarea{\rtail} = \sum_{ (i,k) \in \abs{\cov\pr{\rtail} \setminus \bigcup\limits_{\crule \in \ruleset} \cov\pr{\crule}}  } w_l(k)
\end{equation}

where $w_l(\cdot) : L \rightarrow \mathbb{R}$ is a function mapping each label to a weight. By default the weight is taken to be the complement to $1$ of the relative frequency of a label in the dataset $1-\frac{\dsL}{|\dataset|}$.  

Sampling according to this measure guarantees that less frequent labels are sampled as well. In practice we could introduce an hyperparameter $\alpha$ to control the amount of labels that take into account rarity as well and therefore sample according to $(1-\alpha)\relarea{\rtail} + \alpha \wrelarea{\rtail}$. 

In order to sample according to this varied version of area it is necessary to adjust the weights as follows: 

\begin{align*}
	\sum_{T_1 \in \abs{\relcovR}} \sum_{ (i,k) \in T_1 } w_l(k) 2^{\abs{\covDR}} &=\\ 2^{\abs{\covDR}} \times 2^{\abs{\relcovR}-1} \sum_{ (i,k) \in L_D } w_l(k) &=\\ 2^{|D|-1}  \sum_{ (i,k) \in L_D } w_l(k)
\end{align*}

and then extract from a sampled record $\rtail_1$ with probability: 

\begin{align*}
	\sum_{ (i,k) \in T_1 } w_l(k)
\end{align*}


Plugging-in the above modification in the proof of Proposition~\ref{prop_area_correctness}, it is easy to see that we are sampling according to the desired distribution, i.e., weighted area. 

\cnote[MC]{As an alternative we can sample from the distribution: 

\begin{equation}
	frq^2(T) \prod_{e \in T} ( 1  - frq({e}))
\end{equation}

using e.g. coupling from the past as discussed in~\cite{boley2012linear}
}


\spara{Extreme multi-label classification}
Extending our approach to an extreme multi-label classification setting would be a valuable addition as rule-based XML classification represents a totally unexplored area.
This would mainly require: 
\begin{itemize} 
	\item Improve scalability of our approach 
	
	\item Predict labels ranking (not binary predictions) and use ranking-based evaluation metric 
\end{itemize} 

One approach to tackle the high dimensionality of the label space could be to replace the sampling with a more efficient label clustering technique. To this aim, we assemble the co-occurrence (or correlation) graph for the labels and we run a clustering algorithm over it. Note that this is only needed if the sampling algorithm (and in particular the more scalable CFTP-based version) is to costly to deal with XML setting.   Afterwards, sampling \rhead for each cluster of labels according to discriminative power incurs the same complexity as in the standard setting. However our approach does not output a ranking of the predicted labels but just predicts whether a set of label \rtail is predicted or not as a whole for a given data record. A simple way to solve this issue is by resorting to a post-processing step. Once a rule is sampled, we rank the labels in \rtail according to their confidence measure $\omega(L) = \frac{|\dsL \cap \dsH|}{|\dsH|}$. 

We would then be able to compare our method to other extreme multi-label classifiers using a standard measure such as precision at $k$, thus evaluating the price of interpretability. 

However this approach is not very natural as it is accomplished with a post-processing step. As an alternative we could change our approach to tackle extreme multi-label classification. 
For instance, one can sample rule bodies according to area and diversity and then rank labels according to their confidence. This is trivial to do in polynomial time.  Of course it can be that more rules cover the same instance in which case we could aggregate by averaging the confidence scores so as to obtain a unique ranking. 


A more principled approach is described below. 
We can model the problem of XML classification similarly to the standard multilabel classification problem, but with a relevant difference, i.e. the quality measure. 
A rule \crule defines a label ranking $\ruleRank$ over each $\dr \in \dataset$ which is computed according to the individual label confidence.
We define the quality of a \crule as follows: 

\begin{equation}
	Q(\crule) = \frac{1}{|\dsR|} \sum_{\dr \in \dsR} nDCG(\ruleRank^\dr)
\end{equation}
 
where $nDCG$ is the \emph{normalized discounted cumulative gain}. 

Furthermore, we define a notion of \emph{usefulness}. 
A rule \crule is useful for data record \dr if the associated confidence scores improves the $nDCG$ for that data record. 
Hence, we define the partial (or conditional) benefit of a rule as:  

\begin{equation}
	Q^*(\crule) = \frac{1}{|\dsR|} \sum_{\dr \in \dsR} \mathbf{I} (\useful^{\dr}_{\crule}) \Delta nDCG(\ruleRank^{\dr})
\end{equation}

The role of $\mathbf{I} (\useful^{\dr}_{\crule})$ is to ensure the normalize discounted cumulative gain has a positive increase rather than a negative one. 
Let the total quality of a set be: $\sum_{\crule \in \ruleset} Q(\crule|\ruleset')$.

Furthermore we define as diversity function the Jaccard similarity in the attribute space: 

\begin{equation}
	d(\crule_1, \crule_2) = \frac{|\dsHone \cap \dsHtwo|}{|\dsHone \cup \dsHtwo|}
\end{equation}

and the diversity of a set of rules is defined as $d(\ruleset) = \sum_{\crule_1 \neq \crule_2 \in \ruleset} d(\crule_1, \crule_2)$. 

\begin{problem}
	Given a dataset \dsdef, a budget $\budget\in\integer$, and a parameter $\lambda \in \real_+$, 
	find a set of $\budget$ rules $\ruleset = \set{\crule_1, \ldots, \crule_\budget}$, 
	which maximizes the following objective
	
	\begin{equation}
	\label{eq:obj}
	\sum\limits_{\crule \in \ruleset} Q^*(\crule) + \lambda d(\ruleset),
	\end{equation}
	over the space of all rules \rulespace.
\end{problem}

The problem above is known to be $NP$-hard\cite{zhang2020diverse}. However, as $d(\cdot)$ is a metric and $Q^*(\cdot)$ is a positive monotone submodular set function it follows that we can exploit a $2$-approximation greedy algorithm. 

Clearly as in the standard multi-label classification case we tackle the problem related to the dimension of $\rulespace$ by sampling (diverse) rules according to (uncovered) support or area. 

Note that in the definition of $Q^*(\cdot)$ we do not merge confidence scores of different rules but rather consider a ranking only if it is the best found given the current set of rules. While this may be a (too) simple approach, it does not only guarantee submodularity but also guarantee maximal interpretability.  



==> problem.tex <==
\section{Problem formulation}
\label{sec:prob}






